Multiscale mechanical model based on patient-specific geometry: application to early keratoconus development

Keratoconus is a pathology of the cornea associated with a tissue thinning and a weakening of its mechanical properties. However, it remains elusive which aspect is the leading cause of the disease. To investigate this question, we combined a multiscale model with a patient-geometry in order to simulate the mechanical response of healthy and pathological corneas under intraocular pressure. The constitutive behavior of the cornea is described through an energy function which takes into account the isotropic matrix of the cornea, the geometric structure of collagen lamellae and the quasi-incompressibility of the tissue. A micro-sphere description is implemented to take into account the typical features of the collagen lamellae as obtained experimentally, namely their orientation, their stiffness and their dispersion, as well as the their unfolding stretch, at which they start to provide a significant force. A set of reference parameters is obtained to fit experimental inflation data of the literature. We show that the most sensitive parameter is the unfolding stretch, as a small variation of this parameter induces a major change in the corneal apex displacement. The keratoconus case is then studied by separating the impact of the geometry and the one of the mechanics. We computed the evolution of the SimK (a clinical indicator of cornea curvature) and elevation maps: we were able to reproduce the reported changes of SimK with pressure only by a mechanical weakening, and not by a change in geomtry. More specifically, the weakening has to target the lamellae and not the matrix. The mechanical weakening leads to elevations close to early stage keratoconus, but our model lacks the remodeling component to couple the change in mechanics with changes in geometry.

==> Annexes.tex <==
\section{Computation of the anisotropic $2^{nd}$Piola-Kirchhoff tensor \label{PKtensoraniso_computation_app}}
The transformation is considered as reversible through quasi-static assumption, so the $2^{nd}$ Piola Kirchhoff tensor $\PKstress$ is as in equation \ref{PK_VS_psi}: $\displaystyle \PKstress = 2 \partialderiv{\energyfunction}{\CGtensor}$.

%For the anisotropic part, this translate into equation \ref{PK_aniso_dpsidC}, when decomposing the derivative regarding to the current length of the fiber $l$: $\displaystyle \PKstressaniso  = 2* \partialderiv{\psiAniso}{\CGtensor} = 2* \partialderiv{\psiAniso}{l} \partialderiv{l}{l^2} \partialderiv{l^2}{\CGtensor}$.

For the anisotropic part, this translate into equation \ref{PK_aniso_dpsidC}, when decomposing the derivative regarding to the current length of the fiber $l$: $\displaystyle \PKstressaniso  = 2* \partialderiv{\psiAniso}{\CGtensor} = 2* \partialderiv{\psiAniso}{\elongationfiber} \partialderiv{\elongationfiber}{\elongationfiber^2} \partialderiv{\elongationfiber^2}{\CGtensor}$.

With the energy function defined in equation \ref{psi_aniso_continuous}: \\ 
$\displaystyle \psiAniso \vertjoliwriting{ = \int_{\theta = 0}^{\pi} \int_{\phi = 0}^{2 \pi}{ (\densityfibone \thetaphi \dpsiAnisoone \thetaphi + \densityfibtwo \thetaphi \dpsiAnisotwo \thetaphi) \sin \theta \text{d} \theta  \text{d} \phi} }$

%The only things that depend on $\CGtensor$ and therefore on $l$ in \ref{psi_aniso_continuous} are $\dpsiAnisoone$ and $\dpsiAnisotwo$ and so have to be derived with respect to $l$. Furthermore, terms for fiber one a fiber two are independent so can be treated each independently, so $\dPKstressanisoone$ and $\dPKstressanisotwo$ can be defined as:

%\begin{equation}
%	\begin{cases}
%	\displaystyle \dPKstressanisoone = 2*  \partialderiv{\dpsiAnisoone }{l} \partialderiv{l}{l^2} \partialderiv{l^2}{\CGtensor} \\
%	\displaystyle \dPKstressanisotwo = 2* \partialderiv{\dpsiAnisotwo }{l} \partialderiv{l}{l^2} \partialderiv{l^2}{\CGtensor} \\
%	\end{cases}
%	\label{dPiola_dpsi}
%\end{equation}

The only things that depend on $\CGtensor$ and therefore on $\elongationfiber$ in \ref{psi_aniso_continuous} are $\dpsiAnisoone$ and $\dpsiAnisotwo$ and so have to be derived with respect to $\elongationfiber$. Furthermore, terms for fiber one a fiber two are independent so can be treated each independently, so $\dPKstressanisoone$ and $\dPKstressanisotwo$ can be defined as:

\begin{equation}
\begin{cases}
\displaystyle \dPKstressanisoone = 2*  \partialderiv{\dpsiAnisoone }{\elongationfiber} \partialderiv{\elongationfiber}{\elongationfiber^2} \partialderiv{\elongationfiber^2}{\CGtensor} \\
\displaystyle \dPKstressanisotwo = 2* \partialderiv{\dpsiAnisotwo }{\elongationfiber} \partialderiv{\elongationfiber}{\elongationfiber^2} \partialderiv{\elongationfiber^2}{\CGtensor} \\
\end{cases}
\label{dPiola_dpsi}
\end{equation}


And so $\PKstressaniso$ can be computed with the integral \ref{PK_aniso_continuous_app}:
\begin{equation}
\PKstressaniso =   \vertjoliwriting{ = \int_{\theta=0}^{\pi} \int_{\phi=0}^{2\pi}{(\densityfibone \thetaphi \dPKstressanisoone \thetaphi + \densityfibtwo \thetaphi \dPKstressanisotwo \thetaphi) \sin \theta \text{d} \theta  \text{d} \phi} }
\label{PK_aniso_continuous_app}
\end{equation}

Thanks to the definition of fiber traction $\tractionfibone$ and $\tractionfibtwo$ in \ref{t1_t2_VS_psi1_psi2}, it turns out that:
\begin{center}
$
\begin{cases}
\displaystyle \partialderiv{\dpsiAnisoone}{l} = \tractionfibone  = \stiffnessone ( \frac{ \elongationfiber}{\unfoldingelongationfibone} - 1 )_{+} + \tractionnodfibone \\
\displaystyle \partialderiv{\dpsiAnisotwo}{l} = \tractionfibtwo = \stiffnesstwo (\frac{\elongationfiber}{\unfoldingelongationfibtwo} -1)_{+} + \tractionnodfibtwo
\end{cases}
\text{with} \quad \elongationfiberthetaphi^2 = \rnodthetaphi.\CGtensor.\rnodthetaphi 
$
\end{center}

%The two other useful partial derivative are given in equation \ref{useful_partial_derivative_app}:
%\begin{equation}
%\partialderiv{l}{l^2} = \frac{1}{2l} \quad \text{and}  \quad \partialderiv{l^2}{\CGtensor} = r \otimes r
%\label{useful_partial_derivative_app}
%\end{equation}

The two other useful partial derivative are given in equation \ref{useful_partial_derivative_app}:
\begin{equation}
\partialderiv{\elongationfiber}{\elongationfiber^2} = \frac{1}{2\elongationfiber} \quad \text{and}  \quad \partialderiv{\elongationfiber^2}{\CGtensor} = \rnod  \otimes \rnod 
\label{useful_partial_derivative_app}
\end{equation}


 %The computation for $\displaystyle \partialderiv{l^2}{\CGtensor} = r \otimes r$ in Cartesian coordinates is detailed in equation \ref{dlsquare_dC}. 
 The computation for $\displaystyle \partialderiv{\elongationfiber^2}{\CGtensor} = \rnod \otimes \rnod$ in Cartesian coordinates is detailed in equation \ref{dlsquare_dC}. 
%First the computation of $\lfiberthetaphi$ in Cartesian coordinates is needed, so computed in \ref{elongation_matric_app}.
First the computation of $\elongationfiberthetaphi$ in Cartesian coordinates is needed, so computed in \ref{elongation_matric_app}.
\begin{equation}
\displaystyle \elongationfiberthetaphi^2 = \rnodthetaphi.\CGtensor.\rnodthetaphi = C_{xx} r^2_x + C_{yy}r^2_y +  C_{zz}r^2_z + (C_{xy}+C_{yx}) r_x r_y+  (C_{yz} +C_{zy})r_y r_z+ (C_{xz}+C_{zx}) r_x r_z
\label{elongation_matric_app}
\end{equation}

%\begin{equation}    
%	\displaystyle \partialderiv{l^2}{\CGtensor} = 
%	\begin{pmatrix}
%	\displaystyle \frac{\partial (l^2)}{\partial C_{xx} } & \displaystyle \frac{\partial (l^2)}{\partial C_{xy} } & \displaystyle \frac{\partial (l^2)}{\partial C_{xz} } \\
%	\displaystyle \frac{\partial (l^2)}{\partial C_{xy} } & \displaystyle \frac{\partial (l^2)}{\partial C_{yy} } & \displaystyle \frac{\partial (l^2)}{\partial C_{yz} } \\
%	\displaystyle \frac{\partial (l^2)}{\partial C_{xz} } & \displaystyle \frac{\partial (l^2)}{\partial C_{yz} } & \displaystyle \frac{\partial (l^2)}{\partial C_{zz} } \\
%	\end{pmatrix}
%	=
%	\begin{pmatrix}
%	r^2_x &  r_x r_y &  r_x r_z\\
%	r_x r_y & r^2_y &  r_y r_z\\
%	r_x r_z &  r_y r_z & r^2_z \\
%	\end{pmatrix}
%	= \vect{r} \otimes \vect{r}
%	\label{dlsquare_dC}
%\end{equation}

\begin{equation}    
\displaystyle \partialderiv{\elongationfiber^2}{\CGtensor} = 
\begin{pmatrix}
\displaystyle \frac{\partial (\elongationfiber^2)}{\partial C_{xx} } & \displaystyle \frac{\partial (\elongationfiber^2)}{\partial C_{xy} } & \displaystyle \frac{\partial (\elongationfiber^2)}{\partial C_{xz} } \\
\displaystyle \frac{\partial (\elongationfiber^2)}{\partial C_{xy} } & \displaystyle \frac{\partial (\elongationfiber^2)}{\partial C_{yy} } & \displaystyle \frac{\partial (\elongationfiber^2)}{\partial C_{yz} } \\
\displaystyle \frac{\partial (\elongationfiber^2)}{\partial C_{xz} } & \displaystyle \frac{\partial (\elongationfiber^2)}{\partial C_{yz} } & \displaystyle \frac{\partial (\elongationfiber^2)}{\partial C_{zz} } \\
\end{pmatrix}
=
\begin{pmatrix}
r^2_x &  r_x r_y &  r_x r_z\\
r_x r_y & r^2_y &  r_y r_z\\
r_x r_z &  r_y r_z & r^2_z \\
\end{pmatrix}
= \rnod \otimes \rnod
\label{dlsquare_dC}
\end{equation}


Finally, when everything is assembled, $\dPKstressanisoone$ and $\dPKstressanisotwo$ can be computed as in equation \ref{dPiola_aniso_app}:

%\begin{equation}
%	\begin{cases}
%	\displaystyle \dPKstressanisoone = 2*  \partialderiv{\dpsiAnisoone }{l} \partialderiv{l}{l^2} \partialderiv{l^2}{\CGtensor} =2* \tractionfibone \frac{1}{2l} \rnod \otimes \rnod = (\frac{k}{\elongationfiber l_0} ( \frac{ \elongationfiber}{\unfoldingelongationfibone} - 1 )_{+} + \tractionnodfibone) \rnod \otimes \rnod\\
%	\displaystyle \dPKstressanisotwo = 2* \partialderiv{\dpsiAnisotwo }{l} \partialderiv{l}{l^2} \partialderiv{l^2}{\CGtensor} = \displaystyle 2* \tractionfibtwo \frac{1}{2l} \rnod \otimes \rnod =   (\frac{k}{\elongationfiber l_0} ( \frac{  \elongationfiber}{  \unfoldingelongationfibtwo} - 1 )_{+} + \tractionnodfibtwo) \rnod \otimes \rnod \\
%	\end{cases}
% \label{dPiola_aniso_app}
%\end{equation}



\begin{equation}
\begin{cases}
\displaystyle \dPKstressanisoone = 2*  \partialderiv{\dpsiAnisoone }{\elongationfiber} \partialderiv{\elongationfiber}{\elongationfiber^2} \partialderiv{\elongationfiber^2}{\CGtensor} = 2* \reflenghtfiberone \tractionfibone \frac{1}{2\elongationfiber} \rnod \otimes \rnod = \frac{\reflenghtfiberone}{\elongationfiber}   (\stiffnessone ( \frac{ \elongationfiber}{\unfoldingelongationfibone} - 1 )_{+} + \tractionnodfibone) \rnod \otimes \rnod \\
\displaystyle \dPKstressanisotwo = 2* \partialderiv{\dpsiAnisotwo }{\elongationfiber} \partialderiv{\elongationfiber}{\elongationfiber^2} \partialderiv{\elongationfiber^2}{\CGtensor} = \displaystyle 2* \reflenghtfibertwo \tractionfibtwo \frac{1}{2\elongationfiber} \rnod \otimes \rnod =  \frac{\reflenghtfibertwo}{\elongationfiber}   (\stiffnesstwo ( \frac{  \elongationfiber}{  \unfoldingelongationfibtwo} - 1 )_{+} + \tractionnodfibtwo) \rnod \otimes \rnod \\
\end{cases}
\label{dPiola_aniso_app}
\end{equation}






\section{Computation of the quadrature used in the micro-sphere model \label{quadrature_microsphere_section} }

\subsection{Quadrature used in the FEM code to calculate the  fiber contribution \\}

At each Gauss point, the integral \ref{PK_aniso_app} has to be computed: 
\begin{equation}
	\displaystyle \PKstressaniso   \vertjoliwriting{ = \int_{\theta=0}^{\pi} \int_{\phi=0}^{2\pi}{(\densityfibone \thetaphi \dPKstressanisoone \thetaphi + \densityfibtwo \thetaphi \dPKstressanisotwo \thetaphi) \sin \theta \text{d} \theta  \text{d} \phi} }
	\label{PK_aniso_app}
\end{equation}
In classical FEM code, the tangent computation is needed also. Tangent is the derivative of the 2$^{nd}$ Piola-Kirchhoff tensor with respect to $\GLtensor$, or the 2$^{nd}$ derivative of $\energyfunction$ with respect to $\GLtensor$. With same arguments as in appendix \ref{PKtensoraniso_computation_app}, the tangent can be computed as in equation:

\begin{equation}
\tangentaniso \vertjoliwriting{ = \int_{\theta=0}^{\pi} \int_{\phi=0}^{2\pi}{(\densityfibone \thetaphi \dtangentanisoone \thetaphi + \densityfibtwo \thetaphi \dtangentanisotwo \thetaphi) \sin \theta \text{d} \theta  \text{d} \phi} }
\label{tangent_app}
\end{equation}

Where:

\begin{equation}
\begin{cases}
\displaystyle \dtangentanisoone = 
\begin{cases}
\displaystyle \frac{\stiffnessone - \tractionnodfibone}{\elongationfiber^3} \rnod \otimes \rnod \otimes \rnod \otimes \rnod \quad \text{if} \quad \elongationfiber > \unfoldingelongationfibone \\
\displaystyle \frac{- \tractionnodfibone}{\elongationfiber^3} \rnod \otimes \rnod \otimes \rnod \otimes \rnod \quad \text{if not} \\
\end{cases} \\
\displaystyle \dtangentanisotwo = 
\begin{cases}
\displaystyle \frac{\stiffnesstwo - \tractionnodfibtwo}{\elongationfiber^3} \rnod \otimes \rnod \otimes \rnod \otimes \rnod \quad \text{if} \quad \elongationfiber > \unfoldingelongationfibtwo \\
\displaystyle \frac{- \tractionnodfibtwo}{\elongationfiber^3} \rnod \otimes \rnod \otimes \rnod \otimes \rnod \quad \text{if not} \\
\end{cases} \\
\end{cases}
\label{dtangent}
\end{equation}

First of all, the integrals can be reduced thanks to the invariance in $\pi$ of the density of the fiber in $\phi$:
\begin{center}
$\displaystyle \PKstressaniso   \vertjoliwriting{ = \int_{\theta=0}^{\pi} \int_{\phi=0}^{\pi}{(\densityfibone \thetaphi \dPKstressanisoone \thetaphi + \densityfibtwo \thetaphi \dPKstressanisotwo \thetaphi) \sin \theta \text{d} \theta  \text{d} \phi} }$
\end{center}
and
\begin{center}
	$
\tangentaniso \vertjoliwriting{ = \displaystyle \int_{\theta=0}^{\pi} \int_{\phi=0}^{\pi}{(\densityfibone \thetaphi \dtangentanisoone \thetaphi + \densityfibtwo \thetaphi \dtangentanisotwo \thetaphi) \sin \theta \text{d} \theta  \text{d} \phi} }
$
\end{center}

Then, density functions following the equation \ref{density_functions} recalled below :
\begin{center}
	$\begin{cases}
	\displaystyle \densityfibone \thetaphi = K_1 e^{(\sigma_{p, fib1}\cos(2(\phi-\mu_{fib1})) + \sigma_{t, fib1}\cos(2(\theta-\nu_{fib1})))}, \quad \text{with: } K_1 = \frac{1}{K_{fib1}}  \\
	\\
	\displaystyle \densityfibtwo \thetaphi = K_2 e^{(\sigma_{p, fib2}\cos(2(\phi-\mu_{fib2})) + \sigma_{t, fib2}\cos(2(\theta-\nu_{fib2})))} , \quad \text{with: } K_2 = \frac{1}{K_{fib2}} 
	\end{cases}$
\end{center}

are subject to several assumptions:
\begin{itemize}
	\item the fiber coordinate system is chosen that $\vect{e_x^{fib}}$ coincide with the direction of one fiber. It implies that:  
	\begin{itemize}
		\item $\displaystyle \rho_{fib1} \thetaphi = K_1 e^{\sigma_{p,1}cos(2\phi) + \sigma_{t,1}\cos(2(\theta-\nu_{1})) }$
		\item $\displaystyle \rho_{fib2} \thetaphi = K_2 e^{\sigma_{p,2}\cos(2(\phi+\mu_{1}-\mu_{2})) + \sigma_{t,2}cos(2(\theta-\nu_{2})) }$.
	\end{itemize}
	\item The fiber coordinate system is chosen that the two families of fibers are mainly in the plane $(\exfib,\eyfib)$ (it is in the definition of the coordinates system as $\exfib$ correspond to the first fiber direction and $\eyfib$ correspond to the second fiber direction). It implies that $\nu_1 = \nu_2 = \pi/2$ and so: 
	\begin{itemize}
		\item $\displaystyle \rho_{fib1} \thetaphi = K_1 e^{\sigma_{p,1}\cos(2\phi) + \sigma_{t,1}\cos(2(\theta-\pi/2)) } = K_1 e^{\sigma_{p,1}\cos(2\phi) - \sigma_{t,1}\cos(2\theta) } $
		\item $\displaystyle \rho_{fib2} \thetaphi = K_2 e^{\sigma_{p,2}\cos(2(\phi+\mu_{1}-\mu_{2})) + \sigma_{t,2}\cos(2(\theta-\pi/2)) } = K_2 e^{\sigma_{p,2}\cos(2(\phi+\mu_{1}-\mu_{2})) - \sigma_{t,2}\cos(2\theta) }$.
	\end{itemize}
\end{itemize}

So from now, the integral that needs to be compute is as in equation
\begin{center}
	$\displaystyle \PKstressaniso \textcolor{vertjoli}{= \int_{\theta=0}^{\pi} \int_{\phi=0}^{\pi}K_1 e^{\sigma_{p,1}\cos(2\phi) - \sigma_{t,1}\cos(2\theta) } \dPKstressanisoone +  K_2 e^{\sigma_{p,2}\cos(2(\phi+\mu_{1}-\mu_{2})) - \sigma_{t,2}\cos(2\theta) } \dPKstressanisotwo \sin\theta\text{d}\theta \text{d}\phi}$
\end{center}

and
\begin{center}
	$
	\tangentaniso \vertjoliwriting{ = \displaystyle \int_{\theta=0}^{\pi} \int_{\phi=0}^{\pi}{(K_1 e^{\sigma_{p,1}\cos(2\phi) - \sigma_{t,1}\cos(2\theta) } \dtangentanisoone \thetaphi + K_2 e^{\sigma_{p,2}\cos(2(\phi+\mu_{1}-\mu_{2})) - \sigma_{t,2}\cos(2\theta) } \dtangentanisotwo \thetaphi) \sin \theta \text{d} \theta  \text{d} \phi} }
	$
\end{center}

which can each be decomposed into two parts, which can be treated the same way : 
\begin{itemize}
	\item $\displaystyle \PKstressanisoone = \int_{\theta=0}^{\pi} \int_{\phi=0}^{\pi}K_1 e^{\sigma_{p,1}\cos(2\phi) - \sigma_{t,1}\cos(2\theta) } \dPKstressanisoone \textcolor{vertjoli}{\thetaphi} \sin \theta \text{d} \theta \text{d} \phi$
	\item $\displaystyle \PKstressanisotwo = \int_{\theta=0}^{\pi} \int_{\phi=0}^{\pi}K_2 e^{\sigma_{p,2}\cos(2(\phi+\mu_{1}-\mu_{2})) - \sigma_{t,2}\cos(2\theta) } \dPKstressanisotwo \textcolor{vertjoli}{\thetaphi} \sin \theta \text{d} \theta \text{d} \phi$
	\item $\displaystyle \tangentanisoone = \int_{\theta=0}^{\pi} \int_{\phi=0}^{\pi} K_1 e^{\sigma_{p,1}\cos(2\phi) - \sigma_{t,1}\cos(2\theta) } \dtangentanisoone \textcolor{vertjoli}{\thetaphi} \sin \theta \text{d} \theta \text{d} \phi$
	\item $\displaystyle \tangentanisotwo = \int_{\theta=0}^{\pi} \int_{\phi=0}^{\pi}K_2 e^{\sigma_{p,2}\cos(2(\phi+\mu_{1}-\mu_{2})) - \sigma_{t,2}\cos(2\theta) } \dtangentanisotwo \textcolor{vertjoli}{\thetaphi} \sin \theta \text{d} \theta \text{d} \phi$
\end{itemize}



Quadratures that will be chosen do not depend on the function that changes between the integrals from equation \ref{PK_aniso_app} and \ref{tangent_app} but on those that do not change: the densities $\densityfibone$ and $\densityfibtwo$. Furthermore, the term depending on the two fibers are independent. So, $\PKstressanisoone$ will be chosen as an example, but it is the same with the other terms that we have to compute ($\PKstressanisotwo$, $\tangentanisoone$ and $\tangentanisotwo$).


Here is the computation for $\PKstressanisoone$ :
\begin{center}
	$\displaystyle \PKstressanisoone = \int_{\theta=0}^{\pi} \int_{\phi=0}^{\pi}K_1 e^{\sigma_{p,1}\cos(2\phi) - \sigma_{t,1}\cos(2\theta) } \dPKstressanisoone \textcolor{vertjoli}{\thetaphi}  \sin \theta \text{d} \theta \text{d} \phi$
\end{center}

The integral can be separated in $\theta$ and $\phi$:
\begin{center}
	$\displaystyle \PKstressanisoone= K_1  \int_{\theta=0}^{\pi} e^{ - \sigma_{t,1}\cos(2\theta)} (\int_{\phi=0}^{\pi}e^{\sigma_{p,1}\cos(2\phi)}  \dPKstressanisoone \textcolor{vertjoli}{\thetaphi}  \text{d}\phi) \sin\theta\text{d}\theta$
\end{center}	


\subsubsection{Quadrature in $\phi$ \label{phi_quadrature}\\}
First the integral in $\phi$ of equation \ref{Ione_integral_phi} is considered:

\begin{equation}
\displaystyle I_1 = \int_{\phi=0}^{\pi}e^{\sigma_{p,1}\cos(2\phi)}  \dPKstressanisoone \textcolor{vertjoli}{\thetaphi}  \text{d}\phi
\label{Ione_integral_phi}
\end{equation}	

The function $f_1$ is defined as: $\displaystyle f_1(\phi) = e^{\sigma_{p,1}\cos(2\phi)}  \dPKstressanisoone \textcolor{vertjoli}{\thetaphi} $

and then $I_1$ becomes
\begin{center}
	$\displaystyle I_1 = \int_{\phi=0}^{\pi}f_1(\phi) \text{d}\phi$
\end{center}

For the integral in $\phi$, a uniformly distributed weight is used because a rather smooth distribution of $f_1 = e^{\sigma_{p,1}\cos(2\phi)} \dPKstressanisoone \thetaphi $ in terms of $\phi$ is expected. 

The function is integrated over the segment $[0, \pi]$ with a uniform distribution of the angle $\phi$ : $\displaystyle \forall i \in [1,m], \phi_i = \frac{(i-1)\pi}{m} $, with $m$ the number of equatorial in-plane discretization points.\\
Then, the rectangle method is used to calculate the integral in $\phi$:
\begin{center}
	$\displaystyle I_1 \approx \sum_{i=1}^m (\phi_{i+1}-\phi_i)f_1(\phi_i) \approx \frac{1}{m}  \sum_{i=1}^m f_1(\phi_i) \approx \frac{1}{m}  \sum_{i=1}^m e^{\sigma_{p,1}\cos(2\phi_i)} \dPKstressanisoone \textcolor{vertjoli}{\thetaphii}  $
\end{center}

At this point, $\PKstressanisoone$ is:
\begin{center}
	$\displaystyle \PKstressanisoone = K_1  \int_{\theta=0}^{\pi} e^{ - \sigma_{t,1}\cos(2\theta)} ( \frac{1}{m}  \sum_{i=1}^m e^{\sigma_{p,1}\cos(2\phi_i)} \dPKstressanisoone \textcolor{vertjoli}{\thetaphii} ) \sin\theta\text{d}\theta$
\end{center}

Which can be rearrange and rewrite as:
\begin{center}
	$\displaystyle \PKstressanisoone =  \frac{K_1}{m}  \sum_{i=1}^m e^{\sigma_{p,1}\cos(2\phi_i)}  \int_{\theta=0}^{\pi} e^{ - \sigma_{t,1}\cos(2\theta)}  \dPKstressanisoone \textcolor{vertjoli}{\thetaphii}  \sin\theta\text{d}\theta$
\end{center}

\subsubsection{Quadrature in $\theta$ \label{theta_quadrature}\\ }
Second, the integral in $\theta$ of equation \ref{Itwo_integral_theta} is considered:


\begin{equation}
	\displaystyle I_2 =  \int_{\theta=0}^{\pi} e^{ - \sigma_{t,1}\cos(2\theta)}  \dPKstressanisoone \textcolor{vertjoli}{\thetaphii}  \sin\theta\text{d}\theta
	\label{Itwo_integral_theta}
\end{equation}

The well known trigonometry formula :

\begin{equation}
\displaystyle \cos(2 \theta) = 2\cos^2(\theta) - 1 
\label{trigo_formula}
\end{equation}

help us to rewrite $I_2$ as:

\begin{center}
	$\displaystyle I_2=  \int_{\theta=0}^{\pi} e^{ - \sigma_{t,1}(2\cos^2(\theta) - 1)}  \dPKstressanisoone \textcolor{vertjoli}{\thetaphii}  \sin \theta \text{d} \theta = e^{  \sigma_{t,1}} \int_{\theta=0}^{\pi} e^{ - 2\sigma_{t,1}\cos^2(\theta)} \dPKstressanisoone \textcolor{vertjoli}{\thetaphii} \sin\theta\text{d}\theta$
\end{center}

Then the change of variables of equation \ref{change_variable_theta_x} is applied:

\begin{equation}	
\begin{cases}
\displaystyle 
x = \sqrt{2\sigma_{t,1}}\cos(\theta)\\
\displaystyle 	dx = - \sqrt{2\sigma_{t,1}}\sin(\theta) \\
\end{cases}
\text{and} 
\begin{cases}
\displaystyle \theta = 0 \Leftrightarrow x = \sqrt{2\sigma_{t,1}}\\
\displaystyle \theta = \pi \Leftrightarrow x = - \sqrt{2\sigma_{t,1}}\\
\end{cases}
\label{change_variable_theta_x}
\end{equation}

and the following expression is found for $I_2$:

\begin{center}
	$\displaystyle I_2 =  e^{  \sigma_{t,1}} \int_{x=\sqrt{2\sigma_{t,1}}}^{- \sqrt{2\sigma_{t,1}}} e^{ - x^2}  \dPKstressanisoone \textcolor{vertjoli}{(\arccos(\frac{x}{\sqrt{2\sigma_{t,1}}}),\phi_i) } (- \frac{dx}{\sqrt{2\sigma_{t,1}}})$
\end{center}

The function $f_2$ is defined as: $\displaystyle f_2(x) = \dPKstressanisoone \textcolor{vertjoli}{(\arccos(\frac{x}{\sqrt{2\sigma_{t,1}}}),\phi_i) }$

and then $I_2$ becomes:	
\begin{center}
	$\displaystyle I_2 =  \frac{e^{  \sigma_{t,1}}}{\sqrt{2\sigma_{t,1}}} \int_{x=-\sqrt{2\sigma_{t,1}}}^{ \sqrt{2\sigma_{t,1}}} e^{ - x^2} f_2(x)  dx$
\end{center}		

The Gauss-Hermite quadrature rule gives :
\begin{center}
	$\displaystyle \int_{x= - \infty }^{+ \infty} e^{ - x^2} f(x) dx \approx \sum_{j=1}^{n} \frac{\sqrt{\pi}2^{n+1} n!}{[H_n(x_j)']^2} f(x_j)$
\end{center}	
with $x_j$ the root of the $H_n$ Hermite polynomials which are defined recursively like this:
\begin{center}	
	$
	\begin{cases}
	H_0(x) = 1, H_1(x) = 2x\\
	H_{k+1}(x) = 2x H_k(x) - 2k H_{k-1}(x) \\
	\end{cases}
	$
\end{center}

The function $\overset{\sim}{f_2}$ is defined as follow:
\begin{equation}	
	\begin{array}{ccccc}
	\overset{\sim}{f_2} & : & \mathbb{R} & \to & \mathbb{R}  \\
	& & x & \mapsto & \overset{\sim}{f_2}(x) =  \begin{cases}
	f_2(x) \quad \forall x \in \displaystyle [-\sqrt{2\sigma_{t,1}} ; \sqrt{2\sigma_{t,1}}] \\
	0 \quad \text{elsewhere} \\
	\end{cases}\\
	\end{array}	
	\label{f2tilde}
\end{equation}

Gauss-Hermite approximation is then applied to the $\overset{\sim}{f_2}$ function: 
\begin{center}
	$\displaystyle \int_{x= - \infty }^{+ \infty} e^{ - x^2} \overset{\sim}{f_2} dx \approx \sum_{j=1}^{n} \frac{\sqrt{\pi}2^{n+1} n!}{[H_n(x_j)']^2}  \overset{\sim}{f_2}(x_j)$
\end{center}	

And, so $I_2$ becomes:

\begin{equation}
	\displaystyle I_2 \approx \frac{e^{  \sigma_{t,1}}}{\sqrt{2\sigma_{t,1}}}\sum_{j=1}^{n} \frac{\sqrt{\pi}2^{n+1} n!}{[H_n(x_j)']^2} \overset{\sim}{f_2}(x_j)
	\label{I2_app}
\end{equation}	

Last question that has to be answered is the validity of such an interpolation. The function $\displaystyle \overset{\sim}{f_2}$ is bounded (continue in $x$ on interval $\displaystyle [-\sqrt{2\sigma_{t,1}} ; \sqrt{2\sigma_{t,1}}]$ and equals to 0 elsewhere)

\begin{center}
	$\displaystyle I_2 =  \frac{e^{  \sigma_{t,1}}}{\sqrt{2\sigma_{t,1}}} \int_{x=-\sqrt{2\sigma_{t,1}}}^{ \sqrt{2\sigma_{t,1}}} e^{ - x^2} f_2(x)  dx \leq   \frac{M e^{  \sigma_{t,1}}}{\sqrt{2\sigma_{t,1}}} \int_{x=-\sqrt{2\sigma_{t,1}}}^{ \sqrt{2\sigma_{t,1}}} e^{ - x^2}dx$ 
\end{center}	
with $M$ the maximum of the $\overset{\sim}{f_2}$ function. Now, the integral looks like the integral of a normal distribution.

Here is defined the integral $I_{t,a}$ as the integral of a normal distribution, centered in $0$ on the interval $[-a,a]$ :
\begin{center}
	$\displaystyle I_{t,a} =  \int_{t=-a}^{a} \frac{1}{\sigma \sqrt{2\pi}} e^{ - (\frac{t}{\sqrt{2}\sigma})^2}  dt $ 
\end{center}
For $a = 3 \sigma$, this integral is more than 99 percent of the integral on the whole domain : 

\begin{center}
	$\displaystyle I_{t, 3\sigma}=  \int_{t= -3 \sigma}^{3 \sigma} \frac{1}{\sigma \sqrt{2\pi}} e^{ - (\frac{t}{\sqrt{2}\sigma})^2}  dt  \geq  0.99*I_{t, \infty} = 0.99*  \int_{t= - \infty}^{\infty} \frac{1}{\sigma \sqrt{2\pi}} e^{ - (\frac{t}{\sqrt{2}\sigma})^2}  dt $ 
\end{center}

The following change of variable

\begin{center}	
	$
	\begin{cases}
	\displaystyle u= \frac{t}{\sqrt{2}\sigma}\\
	\displaystyle du = \frac{dt}{\sqrt{2}\sigma} \\
	\end{cases}
	\text{and} 
	\begin{cases}
	\displaystyle t = - 3 \sigma \Leftrightarrow u = -  \frac{3\sqrt{2}}{2}\\
	\displaystyle t =   3 \sigma \Leftrightarrow u = \frac{3\sqrt{2}}{2} \\
	\end{cases}
	$
\end{center}

 is used in $I_{t, 3\sigma}$:

\begin{center}
	$\displaystyle I_{t, 3\sigma} = I_{u, \frac{3\sqrt{2}}{2}}=  \int_{u= - \frac{3\sqrt{2}}{2}}^{ \frac{3\sqrt{2}}{2} } \frac{1}{\sigma \sqrt{2\pi}} e^{ - u^2} \sqrt{2} \sigma du  \geq  0.99 * I_{u, \infty} = 0.99*  \int_{u= - \infty}^{\infty} \frac{1}{\sigma \sqrt{2\pi}} e^{ - u^2}  \sqrt{2} \sigma du$ 
\end{center}

Which can be rewrite as:

\begin{center}
	$\displaystyle  I_{u, \frac{3\sqrt{2}}{2}}=  \frac{1}{ \sqrt{\pi}} \int_{u= - \frac{3\sqrt{2}}{2}}^{ \frac{3\sqrt{2}}{2} } e^{ - u^2}  du  \geq  0.99* I_{u, \infty} = 0.99* \frac{1}{\sqrt{\pi}}  \int_{u= - \infty}^{\infty} e^{ - u^2}  du$ 
\end{center}

Here, a limit value for $\sigma_{t,1}$ that allows to tell that the approximation of $I_2$ by Hermite polynomials is pretty good for all value of $\theta$ can be found:

\begin{center}
	$\displaystyle  \sqrt{2 \sigma_{t,1}} \geq \frac{3\sqrt{2}}{2} \Leftrightarrow  \sigma_{t,1} \geq \frac{9}{4} = 2.25 =  \sigma_{t,min}$ 
\end{center}


Under the assumption of $\sigma_{t,1} \geq  \sigma_{t,min}$, $\PKstressanisoone$ becomes:
\begin{center}
	$\displaystyle \PKstressanisoone \approx  \frac{K_1}{m} \frac{e^{  \sigma_{t,1}}}{\sqrt{2\sigma_{t,1}}}  \sum_{i=1}^m \sum_{j=1}^{n} e^{\sigma_{p,1}\cos(2\phi_i)}\frac{\sqrt{\pi}2^{n+1} n!}{[H_n(x_j)']^2} \overset{\sim}{f_2}(x_j)$
\end{center}

Which can be rearranged as:
\begin{center}
	$\displaystyle \PKstressanisoone \approx  \frac{K_1}{m} \frac{e^{  \sigma_{t,1}}}{\sqrt{2\sigma_{t,1}}}  \sum_{i=1}^m \sum_{j=1}^{n} e^{\sigma_{p,1}\cos(2\phi_i)} \frac{\sqrt{\pi}2^{n+1} n!}{[H_n(x_j)']^2} \textcolor{vertjoli}{\dPKstressanisoonetilde(\arccos(\frac{x_j}{\sqrt{2\sigma_{t,1}}}),\phi_i)}$ 
\end{center}		


And finally:
\begin{center}
	$\displaystyle \PKstressanisoone \approx  \frac{K_1}{m} \frac{e^{  \sigma_{t,1}}}{\sqrt{2\sigma_{t,1}}}  \sum_{i=1}^m \sum_{j=1}^{n} e^{\sigma_{p,1}\cos(2\phi_i)} \frac{\sqrt{\pi}2^{n+1} n!}{[H_n(\sqrt{2\sigma_{t,1}}cos(\theta_j))']^2} \textcolor{vertjoli}{\dPKstressanisoonetilde\thetajphii}$
\end{center}	

In the same way, $\PKstressanisotwo$ can be computed as:
\begin{center}
	$\displaystyle \PKstressanisotwo \approx  \frac{K_2}{m} \frac{e^{  \sigma_{t,2}}}{\sqrt{2\sigma_{t,2}}}  \sum_{i=1}^m \sum_{j=1}^{n} e^{\sigma_{p,2}\cos(2 (\phi_i + \mu_1 - \mu_2))} \frac{\sqrt{\pi}2^{n+1} n!}{[H_n(\sqrt{2\sigma_{t,2}}cos(\theta_j))']^2} \textcolor{vertjoli}{\dPKstressanisotwotilde\thetajphii}$
\end{center}

\subsubsection{Value of $K_1$ and $K_2$\\}

Last thing that has to be known is the values of $K_1$ and $K_2$, which allow that $\rho_{fib1}$ and $\rho_{fib2}$ are density so:
\begin{center}
	$\displaystyle \int_{\theta=0}^{\pi} \int_{\phi=0}^{\pi}\rho_{fib1}(\theta, \phi) \sin\theta\text{d}\theta \text{d}\phi = 1 $ and $\displaystyle \int_{\theta=0}^{\pi} \int_{\phi=0}^{\pi}\rho^M_{fib2}(\theta, \phi)\sin\theta\text{d}\theta \text{d}\phi = 1$
\end{center}

Or rewriting in terms of $K_1$ and $K_2$:

\begin{equation}
\displaystyle \int_{\theta=0}^{\pi} \int_{\phi=0}^{\pi} K_1 e^{\sigma_{p,1}\cos(2\phi) - \sigma_{t,1}\cos(2\theta) } \sin\theta\text{d}\theta \text{d}\phi = 1  \quad \text{and} \quad \int_{\theta=0}^{\pi} \int_{\phi=0}^{\pi} K_2 e^{\sigma_{p,2}\cos(2(\phi+\mu_{1}-\mu_{2})) - \sigma_{t,2}\cos(2\theta) } \sin\theta\text{d}\theta \text{d}\phi = 1 
\end{equation}

And finally, it gives the value of $K_1$ and $K_2$:
\begin{equation}
\displaystyle K_1  =  \frac{1}{\displaystyle \int_{\theta=0}^{\pi} \int_{\phi=0}^{\pi} e^{\sigma_{p,1}\cos(2\phi) - \sigma_{t,1}\cos(2\theta) } \sin\theta\text{d}\theta \text{d}\phi }  \quad \text{and} \quad K_2 = \frac{1}{\displaystyle \int_{\theta=0}^{\pi} \int_{\phi=0}^{\pi} e^{\sigma_{p,2}\cos(2(\phi+\mu_{1}-\mu_{2})) - \sigma_{t,2}\cos(2\theta) } \sin\theta\text{d}\theta \text{d}\phi }
\end{equation}

$K_1$ and $K_2$ computation are equivalent so only one of the two will be considered, and to simplified a bit, the following computation $\frac{1}{K_1}$ will be performed: 
\begin{center}
	$\displaystyle \frac{1}{K_1} = \int_{\theta=0}^{\pi} \int_{\phi=0}^{\pi} e^{\sigma_{p,1}\cos(2\phi) - \sigma_{t,1}\cos(2\theta) } \sin\theta\text{d}\theta \text{d}\phi$
\end{center}

It can decompose in $\theta$ and $\phi$:

\begin{center}
	$\displaystyle \frac{1}{K_1} = \int_{\theta=0}^{\pi} (\int_{\phi=0}^{\pi} e^{\sigma_{p,1}\cos(2\phi)} \text{d}\phi)  e^{- \sigma_{t,1}\cos(2\theta)}  \sin\theta\text{d}\theta $
\end{center}

For the $\phi$ angle, the same rules of quadrature as in \ref{phi_quadrature} is used, and then: 
\begin{center}
	$\displaystyle \frac{1}{K_1} \approx  \int_{\theta=0}^{\pi} (\sum_{i=0}^{m} \frac{1}{m} e^{\sigma_{p,1}\cos(2\phi_i)})  e^{- \sigma_{t,1}\cos(2\theta)}  \sin\theta\text{d}\theta$ with $ \displaystyle \forall i \in [1,m], \phi_i = \frac{(i-1)\pi}{m} $
\end{center}

Or in other terms:
\begin{center}
	$\displaystyle \frac{1}{K_1} \approx  \frac{1}{m} \sum_{i=0}^{m}  e^{\sigma_{p,1}\cos(2\phi_i)}  \int_{\theta=0}^{\pi} e^{- \sigma_{t,1}\cos(2\theta)}  \sin\theta\text{d}\theta$ 
\end{center}

Using the same trigonometry formula \ref{trigo_formula}, the computation gives: 
\begin{center}
	$\displaystyle \frac{1}{K_1} \approx  \frac{1}{m} (\sum_{i=0}^{m}  e^{\sigma_{p,1}\cos(2\phi_i)} ) e^{ \sigma_{t,1}}  \int_{\theta=0}^{\pi} e^{-2\sigma_{t,1}\cos^2(\theta)}  \sin\theta\text{d}\theta$ 
\end{center}

With the same change of variable as in \ref{change_variable_theta_x}, $\displaystyle \frac{1}{K_1}$ becomes:

\begin{center}
	$\displaystyle \frac{1}{K_1} \approx  \frac{1}{m} (\sum_{i=0}^{m}  e^{\sigma_{p,1}\cos(2\phi_i)} ) \frac{e^{ \sigma_{t,1}}}{\sqrt{2\sigma_{t,1}}}  \int_{x = - \sqrt{2\sigma_{t,1}}}^{\sqrt{2\sigma_{t,1}}} e^{-x^2}  \text{d}x$ 
\end{center}

Which is:
\begin{center}
	$\displaystyle \frac{1}{K_1} \approx   \frac{e^{ \sigma_{t,1}}}{m\sqrt{2\sigma_{t,1}}}   \sum_{i=0}^{m}  e^{\sigma_{p,1}\cos(2\phi_i)}  \int_{x = - \sqrt{2\sigma_{t,1}}}^{\sqrt{2\sigma_{t,1}}} e^{-x^2}  \text{d}x$ 
\end{center}

To compute exactly this term, the $erf$ function is needed:
\begin{center}
	$\displaystyle \frac{1}{K_1} \approx   \frac{e^{ \sigma_{t,1}}}{m\sqrt{2\sigma_{t,1}}}   \sum_{i=0}^{m}  e^{\sigma_{p,1}\cos(2\phi_i)} \frac{\sqrt{\pi}}{2} (erf(\sqrt{2\sigma_{t,1}}) - erf(-\sqrt{2\sigma_{t,1}})) \approx   \frac{e^{ \sigma_{t,1}}}{m\sqrt{2\sigma_{t,1}}}   \sum_{i=0}^{m}  e^{\sigma_{p,1}\cos(2\phi_i)} \sqrt{\pi} erf(\sqrt{2\sigma_{t,1}})$ 
\end{center}


%If we do the same hypothesis as in \ref{theta_quadrature} on $\sigma_{t,1}$ to use Gauss-Hermite interpolation, we have then:

%\begin{center}
%	$\displaystyle \frac{1}{K_1} \approx   \frac{e^{ \sigma_{t,1}}}{m\sqrt{2\sigma_{t,1}}}   \sum_{i=0}^{m}  e^{\sigma_{p,1}\cos(2\phi_i)}  \int_{x = - \infty }^{+ \infty} e^{-x^2}  \text{d}x$ 
%\end{center}


%\begin{center}
%	$\displaystyle \frac{1}{K_1} \approx   \frac{e^{ \sigma_{t,1}}}{m\sqrt{2\sigma_{t,1}}}   \sum_{i=0}^{m}  e^{\sigma_{p,1}\cos(2\phi_i)} \sqrt{\pi}$ 
%\end{center}

%\begin{center}
%	$\displaystyle \frac{1}{K_1} \approx   \frac{e^{ \sigma_{t,1}}}{m\sqrt{2\sigma_{t,1}}}   \sum_{i=0}^{m}  e^{\sigma_{p,1}cos(2\phi_i)}  \sum_{j = 1}^{n} \frac{\sqrt{\pi}2^{n+1} n!}{[H_n(\sqrt{2\sigma_{t,2}}cos(\theta_j))']^2}$ 
%\end{center}

%\begin{center}
%$ \displaystyle \frac{1}{K_1} \approx   \frac{e^{ \sigma_{t,1}}}{m\sqrt{2\sigma_{t,1}}}   \sum_{i=0}^{m} \sum_{j = 1}^{n} e^{\sigma_{p,1}cos(2\phi_i)} \lambda_{j,n} \quad \text{with} \quad \forall i \in [1,m], \phi_i = \frac{(i-1)\pi}{m} \quad \text{and} \quad \lambda_{j,n} =\frac{\sqrt{\pi}2^{n+1} n!}{[H_n(\sqrt{2\sigma_{t,2}}cos(\theta_j))']^2}  $
% \end{center}


%\begin{equation}
%\displaystyle {K_1} \approx   \frac{m\sqrt{2\sigma_{t,1}}}{e^{ \sigma_{t,1}}}  \frac{1}{\sum_{i=0}^{m} \sum_{j = 1}^{n} e^{\sigma_{p,1}cos(2\phi_i)} \lambda_{j,n}}   \quad \text{with} 
%\begin{cases}
%\forall i \in [1,m], \phi_i = \frac{(i-1)\pi}{m} \\
%\forall j \in [1,n],  \lambda_{j,n} =\frac{\sqrt{\pi}2^{n+1} n!}{[H_n(\sqrt{2\sigma_{t,2}}cos(\theta_j))']^2}  
%\end{cases}
%\end{equation}

\begin{equation}
\displaystyle {K_1} \approx   \frac{m\sqrt{2\sigma_{t,1}}}{e^{ \sigma_{t,1}}}  \frac{1}{ \sqrt{\pi}erf(\sqrt{2\sigma_{t,1}}) \sum_{i=0}^{m} e^{\sigma_{p,1}\cos(2\phi_i)}}  \quad \text{with} \quad
\forall i \in [1,m], \phi_i = \frac{(i-1)\pi}{m} 
\label{K1_final}
\end{equation}


Reminding the value of $\PKstressanisoone$:
\begin{center}
	$ \displaystyle \PKstressanisoone \approx  \frac{K_1}{m} \frac{e^{  \sigma_{t,1}}}{\sqrt{2\sigma_{t,1}}}  \sum_{i=1}^m \sum_{j=1}^{n} e^{\sigma_{p,1}\cos(2\phi_i)} \frac{\sqrt{\pi}2^{n+1} n!}{[H_n(\sqrt{2\sigma_{t,1}}\cos(\theta_j))']^2} \textcolor{vertjoli}{\dPKstressanisoonetilde\thetajphii}$
\end{center}	

Defining:
\begin{equation}
\displaystyle \forall j \in [1,n],  \lambda_{j,n} = \frac{\sqrt{\pi}2^{n+1} n!}{[H_n(\sqrt{2\sigma_{t,1}}\cos(\theta_j)))']^2} =\frac{\sqrt{\pi}2^{n+1} n!}{[H_n(x_j))']^2}  
\label{weight_Hermite}
\end{equation}

$\PKstressanisoone$ becomes:
\begin{equation}
	\displaystyle \PKstressanisoone \approx  \frac{K_1}{m} \frac{e^{  \sigma_{t,1}}}{\sqrt{2\sigma_{t,1}}}  \sum_{i=1}^m \sum_{j=1}^{n} e^{\sigma_{p,1}\cos(2\phi_i)} \lambda_{j,n} \textcolor{vertjoli}{\dPKstressanisoonetilde\thetajphii} 
	\label{PKstressanisoone_K1}
\end{equation}

Combining \ref{PKstressanisoone_K1} and \ref{K1_final}:
\begin{equation}
\displaystyle  \PKstressanisoone \approx \frac{\displaystyle \sum_{i=1}^m \sum_{j=1}^{n} e^{\sigma_{p,1}\cos(2\phi_i)} \lambda_{j,n} \textcolor{vertjoli}{\dPKstressanisoonetilde\thetajphii} }{\displaystyle \sqrt{\pi} erf(\sqrt{2\sigma_{t,1}}) \sum_{i=1}^m  e^{\sigma_{p,1}\cos(2\phi_i)}}
\quad \text{with} 
\begin{cases}
\displaystyle \forall i \in [1,m], \phi_i = \frac{(i-1)\pi}{m} \\
\displaystyle \forall j \in [1,n], \cos(\theta_{j,k}) = \frac{x_j}{\sqrt{2\sigma_{t,k}}} \\
\text{and} \\
\displaystyle \forall j \in [1,n],  \lambda_{j,n} =\frac{\sqrt{\pi}2^{n+1} n!}{[H_n(x_j))']^2}  
\end{cases}
\end{equation}

%And when, we consider the approximation for the integral in $\theta$:

%\begin{equation}
%\displaystyle  \Psi_{aniso,1}^M \approx  \frac{\displaystyle \sum_{i=1}^m \sum_{j=1}^{n} e^{\sigma_{p,1}cos(2\phi_i)} \lambda_{j,n} \overset{\sim}{\Psi}_{aniso}(\theta_j,\phi_i)}{\displaystyle \sqrt{\pi} \sum_{i=1}^m  e^{\sigma_{p,1}cos(2\phi_i)}}
%\quad \text{with} 
%\begin{cases}
%\displaystyle \forall i \in [1,m], \phi_i = \frac{(i-1)\pi}{m} \\
%\displaystyle \forall j \in [1,n], \cos(\theta_{j,k}) = \frac{x_j}{\sqrt{2\sigma_{t,k}}} \\
%\text{and} \\
%\displaystyle \forall j \in [1,n],  \lambda_{j,n} =\frac{\sqrt{\pi}2^{n+1} n!}{[H_n(x_j)']^2}  
%\end{cases}
%\end{equation}


\subsection{Summary of the quadrature for Piola-Kirchhoff tensor  \label{summary_Piola_Kirchhoff} \\}

To sum up the computation of the 2$^{nd}$ Piola-Kirchhoff tensor:

\begin{equation}
\begin{cases}
\displaystyle  \PKstressanisoone \approx \frac{\displaystyle \sum_{i=1}^m \sum_{j=1}^{n} e^{\sigma_{p,1}\cos(2\phi_i)} \lambda_{j,n} \textcolor{vertjoli}{\dPKstressanisoonetilde\thetajphii} }{\displaystyle \sqrt{\pi} erf(\sqrt{2\sigma_{t,1}}) \sum_{i=1}^m  e^{\sigma_{p,1}\cos(2\phi_i)}}\\
\displaystyle  \PKstressanisotwo \approx \frac{\displaystyle \sum_{i=1}^m \sum_{j=1}^{n} e^{\sigma_{p,1}\cos(2(\phi_i+\mu_{1}-\mu_{2}))} \lambda_{j,n} \textcolor{vertjoli}{\dPKstressanisotwotilde\thetajphii} }{\displaystyle \sqrt{\pi} erf(\sqrt{2\sigma_{t,1}}) \sum_{i=1}^m  e^{\sigma_{p,1}\cos(2(\phi_i+\mu_{1}-\mu_{2}))}}
\end{cases}
\quad \text{with} 
\begin{cases}
\displaystyle \forall i \in [1,m], \phi_i = \frac{(i-1)\pi}{m} \\
\displaystyle \forall j \in [1,n], \cos(\theta_{j,k}) = \frac{x_j}{\sqrt{2\sigma_{t,k}}} \\
\text{and} \\
\displaystyle \forall j \in [1,n],  \lambda_{j,n} =\frac{\sqrt{\pi}2^{n+1} n!}{[H_n(x_j))']^2}  
\end{cases}\\
\label{PKaniso_quadrature}
\end{equation}

%\begin{center}
%	\begin{equation}
%	\begin{cases}
%	\displaystyle  \psiAnisoone \approx  \frac{\displaystyle \sum_{i=1}^m \sum_{j=1}^{n} e^{\sigma_{p,1}\cos(2\phi_i)} \lambda_{j,n} \textcolor{vertjoli}{\overset{\sim}{\dpsiAniso}(\theta_{j,1},\phi_i)} }{\displaystyle \sqrt{\pi} erf(\sqrt{2\sigma_{t,1}}) \sum_{i=1}^m  e^{\sigma_{p,1}\cos(2\phi_i)}} \\
%	\displaystyle  \psiAnisotwo \approx  \frac{\displaystyle \sum_{i=1}^m \sum_{j=1}^{n} e^{\sigma_{p,2}\cos(2\phi_i)} \lambda_{j,n} \textcolor{vertjoli}{\overset{\sim}{\dpsiAniso}(\theta_{j,2},\phi_i)} }{\displaystyle \sqrt{\pi} erf(\sqrt{2\sigma_{t,2}}) \sum_{i=1}^m  e^{\sigma_{p,2}\cos(2\phi_i)}}
%	\end{cases}
%	\quad \text{with} 
%	\begin{cases}
%	\displaystyle \forall i \in [1,m], \phi_i = \frac{(i-1)\pi}{m} \\
%	\displaystyle \forall j \in [1,n], \cos(\theta_{j,k}) = \frac{x_j}{\sqrt{2\sigma_{t,k}}} \\
%	\text{and} \\
%	\displaystyle \forall j \in [1,n],  \lambda_{j,n} =\frac{\sqrt{\pi}2^{n+1} n!}{[H_n(x_j))']^2}  
%	\end{cases}
%	\label{quadrature_microsphere_appendix}
%	\end{equation}
%\end{center}

%Or when, we consider the approximation for the integral in $\theta$:

%\begin{center}
%	\begin{equation}
%	\begin{cases}
%	\displaystyle  \Psi_{aniso,1}^M \approx  \frac{\displaystyle \sum_{i=1}^m \sum_{j=1}^{n} e^{\sigma_{p,1}cos(2\phi_i)} \lambda_{j,n} \overset{\sim}{\Psi}_{aniso}(\theta_{j,1},\phi_i)}{\displaystyle \sqrt{\pi} \sum_{i=1}^m  e^{\sigma_{p,1}cos(2\phi_i)}} \\
%	\displaystyle  \Psi_{aniso,2}^M \approx  \frac{\displaystyle \sum_{i=1}^m \sum_{j=1}^{n} e^{\sigma_{p,2}cos(2\phi_i)} \lambda_{j,n} \overset{\sim}{\Psi}_{aniso}(\theta_{j,2},\phi_i)}{\displaystyle \sqrt{\pi} \sum_{i=1}^m  e^{\sigma_{p,2}cos(2\phi_i)}}
%	\end{cases}
%	\quad \text{with} 
%	\begin{cases}
%	\displaystyle \forall i \in [1,m], \phi_i = \frac{(i-1)\pi}{m} \\
%	\displaystyle \forall j \in [1,n], \cos(\theta_{j,k}) = \frac{x_j}{\sqrt{2\sigma_{t,k}}} \\
%	\text{and} \\
%	\displaystyle \forall j \in [1,n],  \lambda_{j,n} =\frac{\sqrt{\pi}2^{n+1} n!}{[H_n(x_j))']^2}  
%	\end{cases}
%	\label{quadrature_microsphere_approx_theta}
%	\end{equation}
%\end{center}

with  $\forall j \in [1,n], x_j$ the roots of the $H_n$ Hermite polynomials (see table \ref{Hermite_tabular_1_5} for the five first polynomial) which are defined recursively like this:

\begin{center}	
	\begin{equation}
	\begin{cases}
	H_0(x) = 1, H_1(x) = 2x\\
	H_{k+1}(x) = 2x H_k(x) - 2k H_{k-1}(x) \\
	\end{cases}
	\label{Hermite_polynomial_recursive}
	\end{equation}
\end{center}

with $\dPKstressanisoonetilde$ and $\dPKstressanisotwotilde$ defined as in \ref{f2tilde} and $\dPKstressanisoone$ and $\dPKstressanisotwo$ defined as in \ref{dPiola_aniso_final_app}:
\begin{equation}
\begin{cases}
\displaystyle \dPKstressanisoone =  (\frac{k}{\elongationfiber l_0} ( \frac{ \elongationfiber}{\unfoldingelongationfibone} - 1 )_{+} + \tractionnodfibone) \vect{r} \otimes \vect{r} \\
\displaystyle \dPKstressanisotwo =   (\frac{k}{\elongationfiber l_0} ( \frac{  \elongationfiber}{  \unfoldingelongationfibtwo} - 1 )_{+} + \tractionnodfibtwo) \vect{r} \otimes \vect{r} \\
\end{cases}
\text{with} \quad \lfiberthetaphi^2 = \rthetaphi.\CGtensor.\rthetaphi 
\label{dPiola_aniso_final_app}
\end{equation}
%And the function $\overset{\sim}{\Psi}_{aniso}$ defined as follow:
%\begin{center}
%	\begin{equation}
%	\begin{array}{ccccc}
%	 \textcolor{vertjoli}{\overset{\sim}{\dpsiAniso}} & : & \mathbb{R} \quad \text{x} \quad [0, \pi]  & \to & \mathbb{R}^2  \\
%	& & (\theta, \phi) & \mapsto &  \textcolor{vertjoli}{\overset{\sim}{\dpsiAniso}(\theta,\phi)} = 
%	\begin{cases}
% \displaystyle \dpsiAniso \vertjoliwriting{ = \frac{1}{2}k(\lfiberthetaphi - \fiberlnodthetaphi)^2, \quad \forall \theta \in [0, \pi] } \\
%\textcolor{vertjoli}{0	 \quad \text{elsewhere} } \\
%	\end{cases}\\
%	\end{array}	
%	\label{psi_aniso_tilde_appendix}
%	\end{equation}	
%\end{center}

And finally, in the discrete form $\vect{r}$ is given by equation \ref{direction_vector_discrete}: 

%\begin{equation}
%\dpsiAniso \textcolor{vertjoli}{\thetajkphii} = \frac{1}{2}k(\elongationfiber \thetajkphii - \restlenghtfiber)^2 =  \frac{1}{2}k  (\sqrt{\vect{r}(\theta_{j,k}, \phi_i).\tens{C}.\vect{r}(\theta_{j,k}, \phi_i)} - \restlenghtfiber)^2
%\label{discrete_length}
%\end{equation}  
%and 
\begin{equation}
\begin{split}
\vect{r}(\theta_{j,k}, \phi_i) = (\sin\theta_{j,k} \cos\phi_i \exfib(1) + \sin\theta_{j,k} \sin\phi_i \eyfib(1) + \cos \theta_{j,k} \ezfib(1) ) \eX \\ + (\sin\theta_{j,k} \cos\phi_i \exfib(2) + \sin\theta_{j,k} \sin\phi_i \eyfib(2) + \cos \theta_{j,k} \ezfib(2) ) \eY \\ + (\sin\theta_{j,k} \cos\phi_i \exfib(3) + \sin\theta_{j,k} \sin\phi_i \eyfib(3) + \cos \theta_{j,k} \ezfib(3) ) \eZ
\end{split}
\label{direction_vector_discrete}
\end{equation}


\newpage
\section{Five first Hermite polynomials, roots and weight associated  \label{HermitePolynomialAppendix}}

Table \ref{Hermite_tabular_1_5} and \ref{Hermite_tabular_1_5_numerical_value} present the five first Hermite polynomials of order $n$, their roots $ x_{j,n}$ and angles associates $\theta_{j,n}$ for $ \sigma_{t,min} = 2.25$ and weight associated with the roots, first in an explicit form and then with the numerical values.

\begin{table}[h!]
	\begin{tabular}{|c|c|p{3.5cm}|p{4.25cm}|p{4.cm}|}
		\hline
		$n$ & $H_n(x)$ & $x_{j,n}$ : $j$ roots of $H_n(x)$ & $\displaystyle \theta_{j,n} = \arccos(\frac{x_{j,n}}{\sqrt{2\sigma_{t}}})$ with $\sigma_{t} = 2.25$ (in degrees) & $\displaystyle \lambda_{j,n} =  \frac{\sqrt{\pi}2^{n+1} n!}{[H_n(x_j))']^2}= \frac{\sqrt{\pi}2^{n+1} n!}{[H_n(\sqrt{2\sigma_{t}}\cos(\theta_j))']^2}$ \\
		\hline
		$n=1$ & $H_1(x) = 2x$ & $x_{1,1} = 0$ & $\theta_{1,1} = 90 $ & $\displaystyle \lambda_{1,1} = \sqrt{\pi} $ \\
		\hline
		\multirow{2}{*}{$n=2$}  & \multirow{2}{3.5cm}{$H_2(x) = 4x^2 - 2$}  & $\displaystyle x_{1,2} = - \frac{\sqrt{2}}{2} $ & $\theta_{1,2} = 109.471 220 634 504 $ & $\displaystyle \lambda_{1,2} = \frac{\sqrt{\pi}}{2} $ \\ \cline{3-5} && $\displaystyle x_{2,2} = \frac{\sqrt{2}}{2} $ & $\theta_{2,2} = 70.528 779 365 496  $ & $\displaystyle \lambda_{2,2} =  \frac{\sqrt{\pi}}{2} $\\
		\hline
		\multirow{3}{*}{$n=3$}  & \multirow{3}{3.5cm}{$H_3(x) = 8x^3-12x$}  & $\displaystyle x_{1,3} = - \sqrt{ \frac{3}{2}}$ & $\theta_{1,3} = 125.264 389 669 801 $ & $\displaystyle \lambda_{1,3} = \frac{\sqrt{\pi}}{6} $ \\ \cline{3-5} && $x_{2,3} = 0 $ & $\theta_{2,3} = 90 $ & $\displaystyle \lambda_{2,3} = \frac{2\sqrt{\pi}}{3} $ \\ \cline{3-5} && $\displaystyle x_{3,3} =  \sqrt{ \frac{3}{2}} $ & $\theta_{3,3} = 54.735 610 317 232 $ & $\displaystyle \lambda_{3,3} = \frac{\sqrt{\pi}}{6}  $\\
		\hline	
		\multirow{4}{*}{$n=4$}  & \multirow{4}{3.5cm}{$H_4(x) = 16x^4 - 48x^2 +12$}  & $\displaystyle x_{1,4} = - \sqrt{\frac{3+\sqrt{6}}{2}}$ & $\theta_{1,4} = 141. 090 413 810 743 $ & $\displaystyle \lambda_{1,4} = \frac{\sqrt{\pi}(3-\sqrt{6})}{12}  $ \\ \cline{3-5} && $\displaystyle x_{2,4} = - \sqrt{\frac{3-\sqrt{6}}{2}} $ & $\theta_{2,4} = 104.319 054 669 049 $ & $\displaystyle \lambda_{2,4} = \frac{\sqrt{\pi}(3+\sqrt{6})}{12}  $ \\ \cline{3-5} && $\displaystyle x_{3,4} =  \sqrt{\frac{3-\sqrt{6}}{2}}$ & $\theta_{3,4} = 75.680 945 330 951 $ & $\displaystyle \lambda_{3,4} = \frac{\sqrt{\pi}(3+\sqrt{6})}{12}  $ \\ \cline{3-5} && $\displaystyle x_{4,4} =  \sqrt{\frac{3+\sqrt{6}}{2}}  $ & $\theta_{4,4} = 38.909 586 189 258 $ & $\displaystyle \lambda_{4,4} = \frac{\sqrt{\pi}(3-\sqrt{6})}{12} $\\
		\hline
		\multirow{5}{*}{$n=5$}  & \multirow{5}{3.5cm}{$H_5(x) = 32x^5-160x^3+120x$}  & $\displaystyle x_{1,5} = - \sqrt{\frac{5+\sqrt{10}}{2}}$ & $\theta_{1,5} = 162.236 386 701 988  $ & $\displaystyle \lambda_{1,5} = \frac{(7-2\sqrt{10})\sqrt{\pi}}{60} $ \\ \cline{3-5} && $\displaystyle x_{2,5} = - \sqrt{\frac{5-\sqrt{10}}{2}} $ & $\theta_{2,5} = 116.864 071 047 785$ & $\displaystyle \lambda_{2,5} = \frac{(7+2\sqrt{10})\sqrt{\pi}}{60} $ \\ \cline{3-5} && $x_{3,5} = 0$ & $\theta_{3,5} = 90 $ & $\displaystyle \lambda_{3,5} = \frac{8\sqrt{\pi}}{15} $ \\ \cline{3-5} && $\displaystyle x_{4,5} = \sqrt{\frac{5-\sqrt{10}}{2}} $ & $\theta_{4,5} = 63.135 928 952 216 $ & $\displaystyle \lambda_{4,5} = \frac{(7+2\sqrt{10})\sqrt{\pi}}{60}$\\ \cline{3-5} && $\displaystyle x_{5,5} = \sqrt{\frac{5+\sqrt{10}}{2}} $ & $\theta_{5,5} = 17.763 613 298 012 $ & $\displaystyle \lambda_{5,5} = \frac{(7-2\sqrt{10})\sqrt{\pi}}{60}  $\\
		\hline
	\end{tabular}
	\caption{Five first Hermite polynomials of order $\protect n$, roots of the Hermite polynomials $\protect x_{j,n}$ and angles associates $\protect \theta_{j,n}$ for $\protect \sigma_{t,min} = 2.25$ and weight associated with the roots.  \label{Hermite_tabular_1_5} \ccite{greenwood1948}, \ccite{salzer1952} }
\end{table}	

\begin{table}[h!]
	\begin{tabular}{|c|c|p{4.25cm}|p{4.25cm}|p{4.25cm}|}
		\hline
		$n$ & $H_n(x)$ & $x_{j,n}$ : $j$ roots of $H_n(x)$ & $\theta_{j,n} = \arccos(\frac{x_{j,n}}{\sqrt{2\sigma_{t}}})$ with $\sigma_{t} = 2.25$ (in degrees) & $\lambda_{j,n} =  \frac{\sqrt{\pi}2^{n+1} n!}{[H_n(x_j))']^2}= \frac{\sqrt{\pi}2^{n+1} n!}{[H_n(\sqrt{2\sigma_{t}}\cos(\theta_j))']^2}$ \\
		\hline
		$n=1$ & $H_1(x) = 2x$ & $x_{1,1} = 0.000 000 000 000$ & $\theta_{1,1} = 90 $ & $\lambda_{1,1} =  1.772 453 850 906$ \\
		\hline
		\multirow{2}{*}{$n=2$}  & \multirow{2}{2.5cm}{$H_2(x) = 4x^2 - 2$}  & $x_{1,2} = -0.707 106 781 187$ & $\theta_{1,2} = 109.471 220 634 504 $ & $\lambda_{1,2} = 0.886 226 925 453$ \\ \cline{3-5} && $x_{2,2} = 0.707 106 781 187$ & $\theta_{2,2} = 70.528 779 365 496  $ & $\lambda_{2,2} = 0.886 226 925 453$\\
		\hline
		\multirow{3}{*}{$n=3$}  & \multirow{3}{2.5cm}{$H_3(x) = 8x^3-12x$}  & $x_{1,3} = - 1.224 744 871 392$ & $\theta_{1,3} = 125.264 389 669 801 $ & $\lambda_{1,3} = 0.295 408 975 151$ \\ \cline{3-5} && $x_{2,3} = 0.000 000 000 000 $ & $\theta_{2,3} = 90 $ & $\lambda_{2,3} = 1.181 635 900 604$ \\ \cline{3-5} && $x_{3,3} = 1.224 744 871 392 $ & $\theta_{3,3} = 54.735 610 317 232 $ & $\lambda_{3,3} = 0.295 408 975 151 $\\
		\hline	
		\multirow{4}{*}{$n=4$}  & \multirow{4}{2.5cm}{$H_4(x) = 16x^4 - 48x^2 +12$}  & $x_{1,4} = -1.650 680 123 886 $ & $\theta_{1,4} = 141. 090 413 810 743 $ & $\lambda_{1,4} = 0.081 312 835 447 3 $ \\ \cline{3-5} && $x_{2,4} = -0.524 647 623 275  $ & $\theta_{2,4} = 104.319 054 669 049 $ & $\lambda_{2,4} = 0.804 914 090 006 $ \\ \cline{3-5} && $x_{3,4} = 0.524 647 623 275$ & $\theta_{3,4} = 75.680 945 330 951 $ & $\lambda_{3,4} = 0.804 914 090 006 $ \\ \cline{3-5} && $x_{4,4} = 1.650 680 123 886  $ & $\theta_{4,4} = 38.909 586 189 258 $ & $\lambda_{4,4} = 0.081 312 835 447 3$\\
		\hline
		\multirow{5}{*}{$n=5$}  & \multirow{5}{2.5cm}{$H_5(x) = 32x^5-160x^3+120x$}  & $x_{1,5} = -2.020 182 870 456$ & $\theta_{1,5} = 162.236 386 701 988  $ & $\lambda_{1,5} =  0.019 953 242 059 0$ \\ \cline{3-5} && $x_{2,5} = -0.958 572 464 614 $ & $\theta_{2,5} = 116.864 071 047 785$ & $\lambda_{2,5} = 0.393 619 323 152$ \\ \cline{3-5} && $x_{3,5} = 0.000 000 000 000$ & $\theta_{3,5} = 90 $ & $\lambda_{3,5} = 0.945 308 720 483 $ \\ \cline{3-5} && $x_{4,5} = 0.958 572 464 614 $ & $\theta_{4,5} = 63.135 928 952 216 $ & $\lambda_{4,5} = 0.393 619 323 152$\\ \cline{3-5} && $x_{5,5} = 2.020 182 870 456 $ & $\theta_{5,5} = 17.763 613 298 012 $ & $\lambda_{5,5} = 0.019 953 242 059 0$\\
		\hline
	\end{tabular}
	\caption{Five first Hermite polynomials of order $\protect n$, numerical value of the roots of the Hermite polynomials $\protect x_{j,n}$ and numerical value of the angles associates $\protect \theta_{j,n}$ for $\protect \sigma_{t,min} = 2.25$ and numerical value of the weight associated with the roots. \label{Hermite_tabular_1_5_numerical_value} \ccite{greenwood1948}, \ccite{salzer1952} }
\end{table}	

